${S}^5$: The destruction of a bright dwarf galaxy as revealed by the chemistry of the Indus stellar stream

The recently discovered Indus stellar stream exhibits a diverse chemical signature compared to what is found for most other streams due to the abundances of two outlier stars, Indus$\_$0 and Indus$\_$13. Indus$\_$13, exhibits an extreme enhancement in rapid neutron-capture ($r$-)process elements with $\mathrm{[Eu/Fe]} = +1.81$. It thus provides direct evidence of the accreted nature of $r$-process enhanced stars. In this paper we present a detailed chemical analysis of the neutron-capture elements in Indus$\_$13, revealing the star to be slightly actinide poor. The other outlier, Indus$\_0$, displays a globular cluster-like signature with high N, Na, and Al abundances, while the rest of the Indus stars show abundances compatible with a dwarf galaxy origin. Hence, Indus$\_0$ provides the first chemical evidence of a fully disrupted dwarf containing a globular cluster. We use the chemical signature of the Indus stars to discuss the nature of the stream progenitor which was likely a chemically evolved system, with a mass somewhere in the range from Ursa Minor to Fornax.

==> notes.tex <==
Currently three astrophysical environments are considered as potential sources of $r$-process element production in the Universe; neutron star mergers, magneto-rotationally driven supernovae, and collapsars. Theoretical calculations of NSMs has for a long time suggested these as site of heavy element production (lattimer and others). This was confirmed with the detection of the gravitational wave event GW170817 and subsequent multi-wavelength observations of the kilonova xxxx (refs). But there are still many uncertainties regarding the $r$-process element contribution from NSMs to the Galactic chemical evolution. --- more detail? 

Dvorkin et al 2020 find that by implementing turbulent mixing of the NSM ejecta they can explain the observed dispersion in $\mathrm{[Eu/Fe]}$ with $\mathrm{[Fe/H]}$, where as the assembly of the MW from accretion of smaller system has a low impact (That is not really true if the system is not uniformly enriched?). Furthermore, the decreasing trend in $\mathrm{[Eu/Fe]}$ seen in disk stars can also be recreated with an interplay between decreasing star formation rates (decreasing NSM) and increasing type Ia SN contribution.

Holmbeck 2020, did an inverse engineering study deriving the properties if NSM from abundances of r-procsess enhances metal-poor stars assuming NSM are the main enrichment source. From this they find that to create the abundance signature of strongly r-process enhances stars (like Indus 13) highly asymmetric (in mass) binary neutron star pairs are needed, basically to increase the ratio of dynamical ejecta (Dy) compared to disk outflow (Zr). This is not what is observed for the current population of neutron star pairs in the Galaxy. (Put Indus 13 on this map.)


Regular core-collapse supernovae (CCSN) has also been suggested a $r$-process nucleosynthesis sites, however, studies show that the neutrino driven wind of these doesn't become neutron rich enough to produce element much heavier than the first peak (Sr,Y, Zr) (Arcones and others). It is on the other hand possible in a special type of CCSN, the so-called magneto-rotational supernovae (MR-SN), where rotation and strong magnetic fields drive a very asymmetric explosion where neutron-capture nucleosynthesis is shown to happen in jet like outflows. This was first suggested by xxx and the nucleosynthesis yields has been explores in various works since (eg) most recently by Reichert et al. 2020 who find that their model with both rotation and strong magnetic field can produce neutron-capture element up to the third peak (What about actinides? they don't seem to do that.), while models with lower magnetic field produces ejecta a late stages containing elements up to the second peak. 


Collapsars



\subsection{The nature of the Indus stream progenitor}

What do we believe the mass of the Indus stream progenitor was, can it have been something like a classical dwarf spheroidal galaxy which could have had both r-process enhancement and maybe a globular cluster attached? 
The r-process enhanced star can be explained with external pollution for a smaller galaxy or internal but a larger galaxy, the are examples of both small (Grus II) and larger galaxies (UMi) where only a subset of the stars show r-process enhancement. But do a galaxy like UMi also contain cluster like stars? 
How certain are we that IndusXX is actually a steam member? could it come from somewhere else, is it the Jhelum stream there is supposed to be some overlap right?

All of the stars in Indus show some level of $r$-process enhancement and all have [Eu/Ba]>0, make figure with this for all stream stars if not already in Alex paper, this says something about the star formation rate of the systems from which they were stripped. In the MW the s-process sets in around [Fe/H] = -2.5, but it is somewhat later in dwarf galaxies.


%From Nora Shipp 2018 paper
%Indus:
%Length=20.3deg, width= 0.38deg, m-M=16.1, age=13.0Gyr, Z=7*10^-4, number of stars=9700, stellar mass=34*10^3Msun, Mv=-6.2, progenitor mass=650*10^4Msun
%Jehlum:
%Length=29.2deg, width= 1.16deg, m-M=15.6, age=12.0Gyr, Z=9*10^-4, number of stars=4600, stellar mass=13*10^3Msun, Mv=-5.1 progenitor mass=1300*10^4Msun
Metallicity of Indus stream is higher than what would be expected of a system with this magnitude, according to the stellar mass metallicity relation for dwarf galaxies (Kirby 2013)


\subsection{Ursa Minor - possible progenitor}
So far the abundances of the stars in the Indus and Jhelum streams are most similar to those of the Ursa Minor classical dwarf galaxy. 
For stars stars in UMi with high-resolution abundances, 16 stars covering the metallicity range from -1.35 to -3.1 has been analysed by Cohen 2020, Shetrone 2001, ans Sadakane 2004. There is an $\alpha$ present around [Fe/H]= -2 but not going to sub solar alpha abundances before after [Fe/H]0-1.5. The neutron capture abundances all show and $r$-process signature with [Ba/Eu] $\sim$-0.5. There is some spread in the Eu abundances.

Make plot that compares the UMi stars to the Indus / Jhelum stars. 
How does the combined progenitor mass of Indus+Jhelum match that of UMi\?
Compare light elements in COS82 to the Indus star


DISCUSS COMPARISON TO UMI HERE OR REMOVE SECTION
Of the present day intact dwarf galaxies the most natural would be to compare the Indus stream to Ursa Minor
So far the abundances of the stars in the Indus and Jhelum streams are most similar to those of the Ursa Minor classical dwarf galaxy. 
For stars stars in UMi with high-resolution abundances, 16 stars covering the metallicity range from -1.35 to -3.1 has been analysed by Cohen 2020, Shetrone 2001, ans Sadakane 2004. There is an $\alpha$ knee present around [Fe/H]= -2 but not going to sub solar alpha abundances before after [Fe/H]=-1.5. The neutron capture abundances all show and $r$-process signature with [Ba/Eu] $\sim$-0.5. There is some spread in the Eu abundances.


==> obs.tex <==
\begin{rotatetable*}
\begin{deluxetable*}{lccclcccrrrrrrrr}
\centerwidetable
\tablecolumns{16}
\tabletypesize{\scriptsize}
\tablecaption{\label{tab:obs}Observations}
        \tablehead{Name & source\_id & RA & Dec & Obs Date & MJD & $g$ & $r$ & $t_{\text{exp}}$ & Slit & SNR & SNR & $v_{\text{hel}}$ & $\sigma(v)$ & $N_{\text{ord}}$ & $v_{\text{AAT}}$ \\ 
 & & (h:m:s) & (d:m:s) & & & (mag) & (mag) & (min) & (arcsec) & 4500\AA & 6500\AA & (km/s) & (km/s) & & (km/s)} 
\startdata
Indus\_0        & 6390575508661401216 & 23:24:01.75 & $-$64:02:20.8 & 2019-07-27 & 58691.16 & 16.20 & 15.60 &  50 & 0.7 & 25 & 47 &$ -28.8$&  0.2 & 34 &  -28.7 \\ 
Indus\_6        & 6394607108562733440 & 22:56:57.69 & $-$62:41:37.5 & 2019-07-25 & 58689.28 & 17.17 & 16.64 &  90 & 0.7 & 21 & 40 &$ -24.5$&  0.3 & 35 &  -18.2 \\ 
Indus\_8        & 6407002315459841152 & 22:43:18.18 & $-$60:54:22.5 & 2019-07-26 & 58690.21 & 17.37 & 16.83 & 120 & 0.7 & 22 & 41 &$ -42.4$&  0.3 & 13 &  -43.1 \\ 
Indus\_12       & 6411531547451908480 & 22:11:27.25 & $-$58:04:44.7 & 2019-07-26 & 58690.25 & 15.45 & 14.70 &  25 & 0.7 & 24 & 49 &$ -56.2$&  0.3 & 35 &  -58.3 \\ 
Indus\_13       & 6412626111276193920 & 22:05:30.97 & $-$56:30:53.4 & 2019-07-25 & 58689.23 & 17.05 & 16.46 &  86 & 0.7 & 23 & 43 &$ -58.0$&  0.3 & 35 &  -60.2 \\ 
Indus\_14       & 6412885389863009152 & 22:00:10.50 & $-$56:04:10.3 & 2019-07-26 & 58690.18 & 16.64 & 16.01 &  40 & 0.7 & 22 & 42 &$ -65.7$&  0.3 & 35 &  -67.2 \\ 
Indus\_15       & 6461006409605852416 & 21:54:09.09 & $-$55:18:35.0 & 2019-07-28 & 58692.15 & 16.94 & 16.30 &  55 & 0.7 & 21 & 40 &$ -61.1$&  0.3 & 35 &  -62.9 \\ 
\enddata
\end{deluxetable*}
\end{rotatetable*}
